NewsEdits 2.0: Learning the Intentions Behind Updating News

As events progress, news articles often update with new information: if we are not cautious, we risk propagating outdated facts. In this work, we hypothesize that linguistic features indicate factual fluidity, and that we can predict which facts in a news article will update using solely the text of a news article (i.e. not external resources like search engines). We test this hypothesis, first, by isolating fact-updates in large news revisions corpora. News articles may update for many reasons (e.g. factual, stylistic, narrative). We introduce the NewsEdits 2.0 taxonomy, an edit-intentions schema that separates fact updates from stylistic and narrative updates in news writing. We annotate over 9,200 pairs of sentence revisions and train high-scoring ensemble models to apply this schema. Then, taking a large dataset of silver-labeled pairs, we show that we can predict when facts will update in older article drafts with high precision. Finally, to demonstrate the usefulness of these findings, we construct a language model question asking (LLM-QA) abstention task. We wish the LLM to abstain from answering questions when information is likely to become outdated. Using our predictions, we show, LLM absention reaches near oracle levels of accuracy.

==> tables/led_results.tex <==

\begin{table*}[t]
    \small
    \centering
    % \begin{tabular}{|c|c|c|}
    \begin{adjustbox}{max width=0.95\textwidth}
    {
    \begin{tabular}{lrrrrrrrr}
        \toprule
        & \multicolumn{2}{c}{\textbf{All}} & \multicolumn{2}{c}{\textbf{Fact}}& \multicolumn{2}{c}{\textbf{Style}} & \multicolumn{2}{c}{\textbf{Narrative}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
Features &  Macro &  Micro &  Macro &  Micro & Macro &  Micro & Macro & Micro \\
\midrule
Baseline, \textit{fine-grained}                        &      \gca{45.8} &      \gcb{73.6} &           \gcc{32.0} &           \gce{47.2} &            \gcf{58.6} &            \gcg{39.9} &                \gch{52.0} &                \gci{39.9} \\
\midrule
+ NLI                           &      \gca{48.6} &      \gcb{74.1} &           \gcc{45.7} &           \gce{50.4} &            \gcf{55.2} &            \gcg{38.7} &                \gch{43.6} &                \gci{38.7} \\
+ Event                         &      \gca{46.7} &      \gcb{74.1} &           \gcc{39.0} &           \gce{49.0} &            \gcf{59.3} &            \gcg{41.4} &                \gch{41.7} &                \gci{41.4} \\
+ Quote                         &      \gca{46.3} &      \gcb{72.8} &           \gcc{49.8} &           \gce{54.7} &            \gcf{31.9} &            \gcg{28.0} &                \gch{42.4} &                \gci{28.0} \\
+ Collapsed Quote               &      \textbf{\gca{51.2}} &      \gcb{73.9} &           \gcc{38.7} &           \gce{47.6} &            \gcf{58.3} &            \gcg{39.4} &                \gch{51.4} &                \gci{39.4} \\
+ Discourse                     &      \gca{45.8} &      \gcb{75.1} &           \gcc{37.7} &           \gce{49.6} &            \gcf{63.8} &            \gcg{44.6} &                \gch{43.2} &                \gci{44.6} \\
+ Argumentation                 &      \gca{48.9} &      \gcb{73.6} &           \gcc{37.1} &           \gce{47.9} &            \gcf{57.1} &            \gcg{37.7} &                \gch{53.5} &                \gci{37.7} \\
\midrule
+ Discourse \& Event             &      \gca{46.3} &      \gcb{74.3} &           \gcc{38.9} &           \gce{49.9} &            \gcf{62.1} &            \gcg{42.2} &                \gch{42.4} &                \gci{42.2} \\
+ Discourse \& Argumentation     &      \gca{47.8} &      \gcb{74.1} &           \gcc{56.8} &           \gce{50.5} &            \gcf{31.4} &            \gcg{32.2} &                \gch{41.1} &                \gci{32.2} \\
+ Argumentation \& Event         &      \gca{50.0} &      \gcb{75.1} &           \gcc{38.0} &           \gce{48.6} &            \gcf{46.4} &            \gcg{44.9} &                \gch{58.5} &                \gci{44.9} \\
+ Quote \& Discourse             &      \textbf{\gca{51.2}} &      \gcb{72.2} &           \gcc{40.5} &           \gce{45.3} &            \gcf{62.8} &            \gcg{43.0} &                \gch{48.7} &                \gci{43.0} \\
+ Collapsed Quote \& Discourse   &      \gca{49.6} &      \gcb{73.9} &           \gcc{45.6} &           \gce{49.4} &            \gcf{58.9} &            \gcg{39.1} &                \gch{47.9} &                \gci{39.1} \\
+ Collapsed Quote \& NLI         &      \gca{45.4} &      \gcb{72.8} &           \gcc{41.9} &           \gce{50.4} &            \gcf{46.7} &            \gcg{31.2} &                \gch{39.3} &                \gci{31.2} \\
\midrule
+ Collapsed Quote \& NLI \& Event &      \gca{49.0} &      \gcb{73.8} &           \gcc{44.9} &           \gce{48.9} &            \gcf{57.4} &            \gcg{37.0} &                \gch{44.0} &                \gci{37.0} \\
\midrule
+ All                           &      \gca{47.2} &      \gcb{73.6} &           \gcc{40.0} &           \gce{49.7} &            \gcf{58.6} &            \gcg{36.0} &                \gch{43.5} &                \gci{36.0} \\
\midrule 
Baseline, \textit{coarse-grained}   &   49.4 & 56.7 & \multicolumn{2}{c}{46.6}  & \multicolumn{2}{c}{65.1} & \multicolumn{2}{c}{10.4}\\
+ Discourse \& Arg. (Best model, Fact)         &   65.4 & 70.7 & \multicolumn{2}{c}{59.4} & \multicolumn{2}{c}{66.2} & \multicolumn{2}{c}{49.2}\\
\bottomrule
        \end{tabular}
    }
    \end{adjustbox}
    \vspace{-2mm}
    \caption{Various F1 scores (\%) on our test set of the fine-tuned LED model with different combinations of features. Fact/Style/Narrative F1 scores are computed on instances that contain the corresponding labels, whereas All F1 scores are derived from all instances. \looseness=-1}
    \vspace{-5mm}
    \label{tab:led_results}
\end{table*}
% \begin{table*}[t]
%     \small
%     \centering
%     % \begin{tabular}{|c|c|c|}
%     \begin{adjustbox}{max width=0.95\textwidth}
%     {
%     \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Features} & \textbf{Macro F1 (\%)} & \textbf{Micro F1 (\%)} & \textbf{Fact-Type F1 (\%)} & \textbf{Style-Type F1 (\%)} & \textbf{Narrative F1 (\%)}\\
%         \midrule
%         Baseline & \gca{45.8} & \gcb{73.6} & \gcc{32.0} & \gce{58.6} & \gcf{52.0}\\
%         \midrule
%         + NLI & \gca{48.6} & \gcb{74.1} & \gcc{45.7} & \gce{55.2} & \gcf{43.6}\\
%         + Quote & \gca{46.3} & \gcb{72.8} & \gcc{49.8} & \gce{31.9} & \gcf{42.4} \\
%         + Collapsed quote & \textbf{\gca{51.2}} & \gcb{74.0} & \gcc{38.7} & \gce{58.3} & \gcf{51.4}\\
%         + Discourse & \gca{45.8} & \textbf{\gcb{75.1}} & \gcc{37.7} & \gce{60.0} & \gcf{54.5}\\
%         + Argumentation & \gca{48.9} & \gcb{73.6} & \gcc{37.1} & \gce{57.1} & \gcf{53.5}\\
%         + Event & \gca{46.7} & \gcb{74.1} & \gcc{39.0} & \gce{59.3} & \gcf{41.7}\\
%         \midrule
%         + Discourse + Event & \gca{46.7} & \gcb{74.3} & \gcc{38.9} & \gce{64.2} & \gcf{43.9}\\
%         + Discourse + Argumentation  & \gca{47.8} & \gcb{74.1} & \textbf{\gcc{56.9}} & \gce{31.4} & \gcf{41.1}\\
%         + Argumentation + Event & \gca{50.0} & \textbf{\gcb{75.1}} & \gcc{38.0} & \gce{46.4} & \textbf{\gcf{58.5}}\\
%         + Quote + Discourse & \textbf{\gca{51.2}} & \gcb{72.2} & \gcc{40.5} & \textbf{\gce{62.8}} & \gcf{48.7}\\
%         % + Collapse Quote + Discourse & \\
%         + Collapse Quote + NLI & \gca{45.4} & \gcb{72.8} & \gcc{41.9} & \gce{46.7} & \gcf{39.3} \\
%         \midrule
%         + Collapse Quote + NLI + Event & \gca{49.0} & \gcb{73.8} & \gcc{44.9} & \gce{57.4} & \gcf{44.0}\\
%         \midrule
%         + All & \gca{47.3} & \gcb{73.6} & \gcc{40.0} & \gce{58.6} & 43.5\\ 
%       \bottomrule
%         \end{tabular}
%     }
%     \end{adjustbox}
%     \vspace{-2mm}
%     \caption{Various F1 scores on our test set of the fine-tuned LED model with different combination of features.\looseness=-1}
%     \vspace{-5mm}
%     \label{tab:led_results}
% \end{table*}
